WaveStitch: Flexible and Fast Conditional Time Series Generation with Diffusion Models

Generating temporal data under conditions is crucial for forecasting, imputation, and generative tasks. Such data often has metadata and partially observed signals that jointly influence the generated values. However, existing methods face three key limitations: (1) they condition on either the metadata or observed values, but rarely both together; (2) they adopt either training-time approaches that fail to generalize to unseen scenarios, or inference-time approaches that ignore metadata; and (3) they suffer from trade-offs between generation speed and temporal coherence across time windows--choosing either slow but coherent autoregressive methods or fast but incoherent parallel ones. We propose WaveStitch, a novel diffusion-based method to overcome these hurdles through: (1) dual-sourced conditioning on both metadata and partially observed signals; (2) a hybrid training-inference architecture, incorporating metadata during training and observations at inference via gradient-based guidance; and (3) a novel pipeline-style paradigm that generates time windows in parallel while preserving coherence through an inference-time conditional loss and a stitching mechanism. Across diverse datasets, WaveStitch demonstrates adaptability to arbitrary patterns of observed signals, achieving 1.81x lower mean-squared-error compared to the state-of-the-art, and generates data up to 166.48x faster than autoregressive methods while maintaining coherence. Our code is available at: https://github.com/adis98/WaveStitch

==> algorithms/repaintingwavestitch.tex <==
\begin{algorithm}[tb]
\caption{WaveStitch Inference with RePainting}
\label{alg:synthrp}
\begin{algorithmic}[1]

\State \textbf{Input:} 
Windowed metadata ($\mathcal{A}_w$), masks ($\mathcal{M}_w$), and signals ($\mathcal{X}_w$); Timesteps $M$, window size \( w \); Stride \( s \); mini-batch size \(b\); diffusion parameters \( \{ \alpha_t, \beta_t, \overline{\alpha}_t\} \); metadata \( \mathcal{A} = \{\mathbf{a}^{(i)}\}_{i=1}^M \); Denoiser \( f_\theta \).

% \State \textbf{Create windowed samples:}
% \label{ln:windowingrp}
% \vspace{-5pt}
% \[
% \mathcal{X}_w = \{ \mathbf{x}_w^{(i)} = \mathbf{x}^{(i.s - s + 1:i.s -s + w)} \}_{i=1}^{\left\lfloor {(M - w)}/{s} \right\rfloor}, 
% \]
% \[
% \mathcal{A}_w = \{ \mathbf{a}_w^{(i)} = \mathbf{a}^{(i.s - s + 1:i.s -s + w)} \}_{i=1}^{\left\lfloor {(M - w)}/{s} \right\rfloor}, 
% \]
% \[
% \mathcal{M}_w = \{ \mathbf{m}_w^{(i)} = \mathbf{m}^{(i.s - s + 1:i.s -s + w)} \}_{i=1}^{\left\lfloor {(M - w)}/{s} \right\rfloor}, 
% \]

\State \textbf{Initialize outputs:}
\vspace{-5pt}
\[
\mathcal{\hat{X}}_w = \{ \mathbf{\hat{x}}_{w,T}^{(j)}\sim \mathcal{N}(0,I) \}_{j=1}^{\left\lfloor {(M - w)}/{s} \right\rfloor} 
\] 
\vspace{-13pt}
\State \textbf{Divide $\mathcal{X}_w, \mathcal{A}_w, \mathcal{M}_w$ into $(M-w)/(b\times s)$ mini-batches}
% \State \textbf{Initialize output windows:}
% \vspace{-5pt}
% \[
% \mathcal{\hat{X}}_w = \{ \mathbf{\hat{x}}_w^{(i)} = (1-\mathbf{m}_w^{(i)})\cdot \mathbf{x}_w^{(i)} + \mathbf{m}_w^{(i)}\cdot \mathbf{z}^{(i)} \}_{i=1}^{\left\lfloor {(M - w)}/{s} \right\rfloor} 
% \], where \(\mathbf{z}^{(i)}\sim \mathcal{N}(0,I_{w\times C})\)

% \State \textbf{Divide $\mathcal{X}_w, \mathcal{A}_w, \mathcal{M}_w$ into $(M-w)/(b\times s)$ mini-batches}

\For{each mini-batch}
  \For{(\(\mathbf{x}_w^{(j)}, \mathbf{a}_w^{(j)}, \mathbf{m}_w^{(j)}\)) in mini-batch in \textbf{parallel}:}
    \For{step \( t = T, T-1, \dots, 1 \)}
      \State \textbf{Conditional Forward noising}: 
        \label{ln:condfwdnoisingrp}
            \[
            \mathbf{\hat{x}}_{w,t}^{(i)} = (1-\mathbf{m}_w^{(i)})\cdot (\sqrt{\overline{\alpha}_t} \cdot \mathbf{{x}}_w^{(i)} + \sqrt{1 - \overline{\alpha}_t} \cdot \epsilon^{(i)}) + \mathbf{m}_w^{(i)} \cdot \mathbf{\hat{x}}_{w,t}^{(i)}\]
        \vspace{-15pt}
        \State \textbf{One-step denoising}:
        \label{alg:denoisingrp}
        \vspace{-5pt}
        \[
        \mathbf{\hat{x}}_{w,t-1}^{(i)} = \frac{1}{\sqrt{\alpha_t}} \left( \mathbf{\hat{x}}_{w,t}^{(i)} - \frac{1 - \alpha_t}{\sqrt{1 - \overline{\alpha}_t}} \cdot f_{\theta} \left( \mathbf{a}_w^{(i)}, \mathbf{\hat{x}}_{w,t}^{(i)},t \right) \right)
        \]
        \vspace{-10pt}
        \State \textbf{Re-introduce conditions:}
        \[
        \mathbf{\hat{x}}_{w,t-1}^{(i)} = (1-\mathbf{m}_w^{(i)})\cdot \mathbf{x}_w^{(i)}
         + \mathbf{m}_w^{(i)}\cdot \mathbf{\hat{x}}_{w, t-1}^{(i)}\]
      \EndFor
      \If{\(s<w\)}
      \For{\(i > 1\) in \textbf{parallel}}
        \State \textbf{Stitch overlaps:}
    \label{ln:stitchrp}
    \vspace{-5pt}
    \[
    \mathbf{\hat{x}}_w^{(i)(1:w-s)} = \mathbf{\hat{x}}_w^{(i-1)(1+s:w)}
    \]
    \vspace{-15pt}
    \EndFor
    \EndIf
  \EndFor
\EndFor

\State \textbf{Merge windows:}
\vspace{-5pt}
\[
\mathcal{\hat{X}} = \mathbf{\hat{x}}_w^{(1)} \cup 
\left(
\bigcup_{i\geq 2} \mathbf{\hat{x}}_w^{(i)(w-s+1:w)}
\right)
\]
\vspace{-10pt}
\State \Return {\(\mathcal{\hat{X}}\)}

\end{algorithmic}
\end{algorithm}





==> sections/method.tex <==
\section{\algo}
\input{tables/notation}

% \lc{Stress why gradient based conditional synthesis, not repainting. We need to provide pros and cons for these two methods (in related work)2. Stress why stitch loss is so unique to the time series, but NOT for images Argue for its generalization. 3. In the evaluation, we stress we have both approaches}

This section defines our problem, laying \algo's foundation, which employs diffusion models to generate conditional time-series signals. Then, we detail our mechanisms for tackling key challenges: flexibly handling inference-time conditions, enabling parallel sequence generation, and  \lc{change the following?}implementing temporal encoding schemes.

% \lc{I am goign to rewrite the first part of section 3.1 and 3.2. I find those examples very convoluted. We just need figure 4}
\subsection{Problem Definition}
% \lc{For me, the problem defintiion is the "inference" problem, and what training data is given. I will modify }
We are given a time series dataset as
\(
\mathcal{D} = \{(\mathbf{a}^{(i)}, \mathbf{x}^{(i)})\}_{i=1}^N,
\)
where $\mathbf{a}^{(i)}\in \mathbb{R}^{1\times L}$ denotes the auxiliary $L$ features and $\mathbf{x}^{(i)}\in \mathbb{R}^{1\times C}$ is the $C$-variate signal at timestep \(i=\{1, \dots N\}\).  %The auxiliaries are represented by the dataset \(\mathcal{A} = \{\mathbf{a}^{(i)}\}_{i=1}^N\), where $\mathbf{a}^{(i)}\in \mathbb{R}^{1\times L}$ , consist of $L$ features and $N$ timesteps.% Similarly, the multivariate signal dataset is $\mathcal{X} = \{\mathbf{x}^{(i)}\}_{i=1}^N$, where $\mathbf{x}^{(i)}\in \mathbb{R}^{1\times C}$, consists of $C$ channels per timestep.
The aim is to generate a new set of time series, given any combinations of auxlimiary features and singal anchors.
We assume that full time series dataset \(\mathcal{D}\), including auxiliary features and singal patterns are available during the training. 
%\{(\mathbf{a}^{(i)}, \mathbf{x}^{(i)})\}_{i=1}^N\), consisting of auxiliary values \(\mathbf{a}^{(i)}\) and signal \(\mathbf{x}^{(i)}\) across \(i=\{1 \dots N\}\) timesteps.
However, during inference, we are given a condition that partially specifies the values of the auxiliary feature vector, which essentially differ from the model training  inputs.
For example, a condition such as $\mathbf{a}^{(k)} = (\text{val}_1, \text{val}_2, *, *, *)$ indicates that on needs to generate signal values for all timesteps $k$ where the first two auxiliary features match $\text{val}_1$ and $\text{val}_2$, regardless of the remaining values. The asterisk ($*$) denotes that no constraint is applied to that feature.

To construct the set 
$\{\mathbf{a}^{(k)}\}$, we enumerate all valid combinations of the unspecified features observed during training, yielding auxiliary vectors that satisfy the given condition. These auxiliary vectors are then inserted into 
$\mathcal{D}$ at their appropriate positions in the timeline\footnote{Duplicate entries are not added since they are already present in $\mathcal{D}$}. Then, we generate the signal values $\mathbf{x}^{(k)}$ by conditioning on $\mathbf{a}^{(k)}$ and the signal anchors $\mathbf{x}^{(i)}$ from other timesteps $i \neq k$. We further illustrate the problem of conditioning on auxiliary features and signal anchors in the following example and \autoref{fig:constraintfigure}.
%To illustrate this setup, consider the following example.

\begin{myframe}[innerleftmargin = 5pt]
\label{exmp:2}
\bemph{Example 1.} Consider a dataset containing one year’s worth of daily sales data for three brands---\textit{A}, \textit{B}, and \textit{C}. Each Sales entry (signal) is associated with the auxiliaries {Brand}, {Month}, and {Day}. The data is organized by concatenating the entries from all three brands into a single table. Each row corresponds to a unique combination of (Brand, Month, Day), and is assigned a timestep index based on its row position. 

Consider a condition at the root auxiliary, such as \( (\text{\emph{Brand}}=B, *, *) \)---requiring the generation of sales values for the entire year for Brand \textit{A}. The signal positions needing generation are shown in \autoref{fig:year}. Here, we see that, the generated portions comprise a long \emph{contiguous block} of signal timesteps---the granularity is \emph{coarse-grained}. 

Now consider a constraint applied at the last auxiliary feature, such as \((*, *, \text{\emph{Day}}=15) \), with the brand and month variable. Here, we need to generate sales values for the $15^{\text{th}}$ day of each month for all three brands. Unlike the earlier task, the generated signals are not temporal neighbours, as shown in \autoref{fig:day}. Thus, this conditioning resembles \emph{fine-grained} tasks where the generated values are dispersed across timesteps. 
% \end{mdframed}
\end{myframe}

% \begin{mdframed}
% \begin{myframe}[innerleftmargin = 5pt]
% \bemph{Example 1:} Consider the table in \autoref{fig:arbitconst} and the constraint $(B,X,*)$. The problem is to generate the revenue values for the matching rows $(B,X,2017), (B,X,2018),$ and $(B,X,2019)$, by feeding them as auxiliary conditions along with the historical signals, such as revenues from $(A,Y,2017/2018)$ and $(B,Y,2017/2018)$.
% % \end{mdframed}
% \end{myframe} 



\begin{figure*}[t]
    \centering
    \begin{subfigure}{0.3\textwidth}
    \includegraphics[width=\textwidth]{images/c.drawio.pdf} 
    \caption{Auxiliary Condition: $(B, *, *)$}
    \label{fig:year}
    \end{subfigure}
    \begin{subfigure}{0.3\textwidth}
    \includegraphics[width=\textwidth]{images/m.drawio.pdf}  
    \caption{Auxiliary Condition: $(*, {January}, *)$}
    \label{fig:month}
    \end{subfigure}
    \begin{subfigure}{0.3\textwidth}
    \includegraphics[width=\textwidth]{images/f.pdf}
    \caption{Auxiliary Condition: $(*, *, 15)$}
    \label{fig:day}
    \end{subfigure}
    \caption{Illustration of Synthesised Timesteps Matching Different Types of Auxiliary Conditions In \hyperref[exmp:2]{Example 1}.}
    \label{fig:constraintfigure}
\end{figure*}
\subsection{Conditional Time Series Synthesis}
\label{subsec:dynamic}

% \lc{I comment out the example 2. Because I think figure 4 is sufficient. We can put it back if needed}



% While \hyperref[exmp:2]{Example 2} considers auxiliary conditions at the root and bottom levels, we may also impose conditions at intermediate levels, like \autoref{fig:month}, or across multiple levels. The key point is that conditions at different levels affect the \emph{degree of missingness} and the \emph{conditional mask}~\cite{alcaraz2022diffusion}, which indicates the timesteps of the historical (conditional) signals and the ones requiring generation. As discussed in \autoref{subsec:conditionalddpm}, training time solutions like SSSD~\cite{alcaraz2022diffusion} are not scalable. They require training separate models for each constraint type and proportion of missing signal values~\cite{alcaraz2022diffusion}. Thus, we advocate for the handling the conditioning at \emph{inference time}, inspired by methods like RePaint~\cite{lugmayr2022repaint}, TSDiff~\cite{kollovieh2024predict}, and RelDDPM~\cite{liu2024controllable}. This removes the dependence on specific conditional masks or missingness patterns, allowing for flexibility during generation.  


% Training a model that conditions on available signal values may improve the accuracy during generation. However, this approach is unreliable during inference because we cannot predetermine which parts of the signal will be available. This is because the positions of the conditional (available) signals are set based on the auxiliary constraint at inference time, as shown in \autoref{fig:constraintfigure}. 
% \lc{i will ddd one paragraph on the overview of the parallel stitch}
{
From \hyperref[exmp:2]{example 1} and \autoref{fig:constraintfigure}, we see that the positions of the observed anchors (in green) and the ones needing generation (in red) can vary significantly depending on the auxiliary condition provided. It is impossible to know beforehand  the combined pattern of anchors and values-to-generate at during inference. We thus design \algo combining the training and inference time conditions to agilely handel diversified  condition patterns. 

Specifically, the \algo is composed of two components: the training of auxiliary-conditioned denoiser and singal-conditioned inference. We first train a multi-variate time series denoiser $f_\theta$ to estimate the noise using \textit{only} the auxiliary features, % $\mathcal{A}$,
without making assumptions about the anchor positions during inference. During the inference time,  we iteratively generate the samples based on the given auxiliary and singal conditions. Different from the standard denoising process,  we first generate the denoised sample and then correct this estimate using the gradient from our novel conditional loss on the observed anchors. This design of iterative correcting the denoised samples is inspired from the gradient inversion attack~\cite{jeon2021gradient}, which samples are iteratively adjusted based on the gradient of current loss values. After every denoising step using the auxiliary-conditioned desnoiser, we ajdjust the samples such that the singal anchor conditions are taken into consideration. 

%In the \textit{worst case}, we may have no signal anchors available at inference---training such an \textit{auxiliary-only} conditional denoiser prepares the model to handle this bare minimum setting. \emph{Our method dynamically incorporates these anchors at inference is detailed in the following subsection}.


.

\input{algorithms/training}
\subsubsection{Training Auxiliary-conditioned denoiser}
Our training process is illustrated in \autoref{fig:training} and detailed in \hyperref[alg:training]{Algorithm 1}. It begins with dividing the entire dataset sequence of $N$ timesteps into overlapping windows of size $w$ (line \ref{alg:trainingwindow}), using a stride of one. Then, we noise the window up to a randomly sampled diffusion step $t$ and estimate the added noise, following the standard DDPM training process~\cite{ho2020denoising} (lines \ref{ln:fwdnoise},\ref{ln:estimatenoise}). The noise is estimated by conditioning on the full set of auxiliary features for the window, $\mathbf{a}^{(i:i+w-1)}$, and the mean-squared-error (MSE) loss is used to update $f_\theta$'s parameters (line \ref{ln:loss}). This allows the model to learn the interactions between the auxiliaries and the signals without relying on any signal anchors. However, as discussed earlier, conditioning on the anchors during inference can enhance generation quality---especially for finer-grained tasks like in \autoref{fig:day}---where timesteps requiring generation can be estimated using the neighbouring anchors.}

\input{algorithms/pipelining}
% TimeWeaver~\cite{narasimhan2024time} also follows this training process and operates similarly during inference without conditioning on the available signals. However, \algo conditions on neighboring signal values \emph{and} auxiliary features during inference, improving generation accuracy. This is especially true for fine-grained tasks like \autoref{fig:day}, where neighboring conditional signal values substantially help in predicting the missing parts.

% Since 
% $f_\theta$ only conditions on auxiliary features, we need to condition on the available signal values during inference, which we implement in \hyperref[alg:synth]{Algorithm 2}. To condition on the values within a window, we 
{


% \subsubsection{Conditional Denoising with the Gradient of Conditional Loss}. \lc{I will add a few sentences. We also need a reason for our pre processing}
\subsubsection{Inferencing.} Our process for conditional generation at inference consists of several steps, which we detail as follows:

\textbf{1. Pre-processing.}  \lc{pre-processing shall be bfore the training?}We define the test set \( \mathcal{X} = \{ \mathbf{x}^{(i)} \}_{i=1}^M \), where \( \mathbf{x}^{(i)} \) contains the known historical signals at the observed timesteps, and the unknown values are left empty, representing the portions to be generated. The complete set of auxiliaries, \( \mathcal{A} = \{ \mathbf{a}^{(i)} \}_{i=1}^M \), is also available and provides additional conditioning information. A corresponding mask \( \mathcal{M} = \{ \mathbf{m}^{(i)} \}_{i=1}^M \) is defined, where \( \mathbf{m}^{(i)} = 1 \) indicates that \( \mathbf{x}^{(i)} \) requires generation and \( \mathbf{m}^{(i)} = 0 \) marks the anchors. We first divide the test set into overlapping time windows of size \( w \), spaced by a stride \( s \), yielding \( \mathcal{X}_w = \{ \mathbf{x}_w^{(j)} \}_{j=1}^{\left\lfloor \frac{M - w}{s} \right\rfloor} \), \( \mathcal{M}_w = \{ \mathbf{m}_w^{(j)} \}_{i=j}^{\left\lfloor \frac{M - w}{s} \right\rfloor} \), and \( \mathcal{A}_w = \{ \mathbf{a}_w^{(j)} \}_{i=j}^{\left\lfloor \frac{M - w}{s} \right\rfloor} \). Following this, we proceed with the generation process, detailed  in  \hyperref[alg:synth]{Algorithm 2}, which iterates through steps of $t=T,T-1 \dots 1$ to first generate the denoised sample using the trained denoiser and then adjust the sample by the gradient of the conditional loss for the signal alignment.  

\textbf{2. Auxiliary-Conditioned Generation.}
We first initialize the signal to be generated ($\mathcal{\hat{X}}_w$) in line \ref{ln:init}. Then we divide $\mathcal{X}_w$, $\mathcal{M}_w$, and $\mathcal{A}_w$ into mini-batches of size $b$, each containing samples of $w$ timesteps (line \ref{ln:mini}). To condition on available signals \textit{and} auxiliaries, we first get a dirty estimate of the fully-denoised signal ($\mathbf{\hat{x}}_{w,0}^{(j)}$) using our auxiliary-conditioned denoiser. This is achieved by reversing the fast-forward noising step Eq.~\eqref{eq:ffwdnoising} as follows :
\begin{equation}
\label{eq:dirtyestimate}
    \mathbf{\hat{x}}_{w,0}^{(j)} = 
    % \frac{1}{\sqrt{\alpha_t}} \left( \mathbf{\hat{x}}_{w,t}^{(j)} - \frac{1 - \alpha_t}{\sqrt{1 - \bar{\alpha}_t}} \cdot f_{\theta} \left( \mathbf{a}_w^{(j)}, \mathbf{\hat{x}}_{w,t}^{(j)},t \right) \right) 
    \frac{\mathbf{\hat{x}}_{w,t}^{(j)} - \sqrt{1-\bar{\alpha}_t} \cdot f_{\theta} \left( \mathbf{a}_w^{(j)},    \mathbf{\hat{x}}_{w,t}^{(j)},t \right)}{\sqrt{\bar{\alpha}_t}} 
\end{equation}

Here, $\mathbf{\hat{x}}_{w,t}^{(j)}$ refers to the $j\textsuperscript{th}$ sample window estimate at the $t\textsuperscript{th}$ diffusion step. 

\textbf{3. Sample adjustment with gradient inversion.}
The denoiser $f_{\theta}$ estimates samples  by only conditioning on the auxiliaries. To further factor in the observed signal values, we correct the samples using the gradients w.r.t a conditional loss.  
This conditional loss combines two loss terms, namely the \textit{self-guidance} loss and \textit{stitch} loss, which ensure the coherence within and across time windows, respectively.}
 %By combining the self-guidance loss and stitching loss, 
Specifically, we let the  conditioning loss:

\begin{equation}
\label{eq:finalcondloss}
\mathcal{L}^{(j)} = \mathcal{L}_{\text{self}}^{(j)} + \mathcal{L}_{\text{stitch}}^{(j)}
\end{equation}

%{We adjust the input samples using gradient information with respect to the provided signals. This is where the core conditioning process takes place, ensuring that the generated signal is aligned with the available data.} Specifically, we adjust the input samples using gradient information, while keeping the denoiser's backbone frozen, similar to \textit{gradient inversion}~\cite{jeon2021gradient,huang2021evaluating}. However, unlike standard gradient inversion, which applies the same loss function used during the denoiser's training, we introduce a customized loss function tailored for time series generation.

\emph{Self-guidance loss}.
To ensure the generated signal values aligning with the observed signals within the same window, we need to condition on the observed signal values within a given time window. To such an end, we introduce the self-guidance loss~\cite{kollovieh2024predict}:

\begin{equation}
\mathcal{L}_{\text{self}}^{(j)} = \|(1 - \mathbf{m}_w^{(j)}) \odot (\mathbf{\hat{x}}_{w,0}^{(j)} - \mathbf{x}_{w}^{(j)})\|^2,
\end{equation}

This loss essentially quantifies the mean square errors between the predicted values and the given conditional values.
%However, as the name suggests, self-guidance only constrains the signal values to align with the observed signals within the same window. 

\emph{Stitch loss}. Since the self-guidance loss considers each window independently, it fails to account for the important overlap between consecutive windows.
In time series data, the overlapping regions between windows carry critical information that ensures the continuity and coherence of the sequence. Without considering this overlap, different parts of the sequence may not align properly, leading to incoherencies where the windows meet.

To address this, we introduce the \textit{stitching loss}, which minimizes discrepancies in the overlapping regions between consecutive windows. For a given window \( \mathbf{\hat{x}}_{w,t}^{(j)} \), and its predecessor \( \mathbf{\hat{x}}_{w,t}^{(j-1)} \), the overlap consists of the first \( w - s \) timesteps of \( \mathbf{\hat{x}}_{w,t}^{(j)} \) and the last \( w - s \) timesteps of \( \mathbf{\hat{x}}_{w,t}^{(j-1)} \). Rather than synthesizing these regions independently, we enforce coherence by minimizing the discrepancy between the overlapping regions:

\begin{equation}
\mathcal{L}_{\text{stitch}}^{(j)} = \|\mathbf{\hat{x}}_{w,t}^{(j)(1:w-s)} - \mathbf{\hat{x}}_{w,t}^{(j-1)(1+s:w)}\|^2
\end{equation}

For the first window, we define \( \mathcal{L}_{\text{stitch}}^{(1)} = 0 \), as there are no preceding windows.  

\emph{Adjustment}. To incorporate these constraints into the generation process, we first perform a standard unconditional denoising step using Eq.~\eqref{eq:initguess}, like Eq.~\eqref{eq:denoiseone} in \autoref{subsec:diffforts}. Then, we adjust it using the gradient scaled by guidance strength \(\eta\) using Eq.~\eqref{eq:onestepconditden}, as follows:
\begin{equation}
    \label{eq:initguess}
    \mathbf{\hat{x'}}_{w,t-1}^{(j)} = \frac{1}{\sqrt{\alpha_t}} \left( \mathbf{\hat{x}}_{w,t}^{(j)} - \frac{1 - \alpha_t}{\sqrt{1 - \bar{\alpha}_t}} \cdot f_{\theta} \left( \mathbf{a}_w^{(j)}, \mathbf{\hat{x}}_{w,t}^{(j)},t \right) \right)  
    + \sigma_t z
\end{equation}

\begin{equation}
\label{eq:onestepconditden}
    \mathbf{\hat{x}}_{w,t-1}^{(j)} = \mathbf{\hat{x'}}_{w,t-1}^{(j)}
    %\frac{1}{\sqrt{\alpha_t}} \left( \mathbf{\hat{x}}_{w,t}^{(j)} - \frac{1 - \alpha_t}{\sqrt{1 - \bar{\alpha}_t}} \cdot f_{\theta} \left( \mathbf{a}_w^{(j)}, \mathbf{\hat{x}}_{w,t}^{(j)},t \right) \right)  
     - \eta \nabla_{\mathbf{\hat{x}}_{w,t}^{(j)}} \mathcal{L}^{(j)}
\end{equation}

Similar to Eq.~\eqref{eq:denoiseone}, $z\sim \mathcal{N}(0,I)$, and $\sigma_t = (1-\alpha_t)\frac{1-\bar{\alpha}_{t-1}}{1-\bar{\alpha}_t}$. At the end of the denoising process, we reintroduce the historical signals (line \ref{ln:reint}) and merge the sliding windows (line \ref{ln:merge}), ensuring that the generated signal is coherent across the entire sequence. We illustrate the conditional denoising process using the combination of the two losses in \autoref{fig:stitch}.




% We first apply a conditional mask to estimate noised versions of the available signals, as illustrated in step 1 of \autoref{fig:repainting} and implemented in line \ref{ln:condfwdnoising}. This mask is a binary vector with ones indicating the values for the timesteps to generate. After this, the denoising process is applied to the entire signal (line \ref{alg:denoising}). Conditions are then re-introduced before the next iteration. At each denoising step, the known signal parts influence the unconstrained portions to naturally adjust in a way that remains consistent with the overall signal pattern. This way, we can produce a coherent signal that jointly conditions on both the auxiliary features and historical signals at inference time.

\begin{figure}[tb]
    \centering
      \includegraphics[width=0.45\textwidth]{images/training.drawio.pdf}
    \caption{Auxiliary-conditioned Denoiser Training}
    \label{fig:training}
\end{figure}
\begin{figure*}[tb]
    \centering
      \includegraphics[width=\textwidth]{images/syntha1.drawio.png}
    \caption{Parallel Inference-conditioning with Stitch and Self-Guidance Loss. At each step $t$, the gradients for the stitching loss (in \textcolor{orange}{orange}) and the self-guidance loss (in \textcolor{blue}{blue}) are combined to refine the initial auxiliary-conditioned estimate.}
    \label{fig:stitch}
\end{figure*}
% \begin{figure*}[tb]
%     \centering
%     \includegraphics[width=\textwidth]{images/syntha.drawio.pdf}
%     \caption{Conditional Denoising and Parallel Denoising of Overlapping Windows with Stitching}
%     \label{fig:inferencetricks}
% \end{figure*}

\subsection{ Parallel Generation}
{
The conditioning mechanism described in \autoref{subsec:dynamic} could be applied autoregressively by processing each window sequentially. However, we observe that most operations can be performed independently for each window, enabling efficient parallelization. The only operation that introduces dependencies between windows is the stitching loss. However, this step can also be parallelized, as shown in \hyperref[alg:synth]{Algorithm 2}. This can be done in a single batched operation by performing a \emph{shift} (or roll) of all windows and aligning the overlaps of each window with the rolled version. This process resembles a \emph{pipeline}---although dependencies are enforced only with the immediately preceding window, coherence emerges gradually over successive denoising iterations. As information propagates through the overlaps, non-overlapping parts adjust to maintain coherence with their neighbours, ultimately leading to global consistency. 
}

The stride \( s \) is crucial in balancing efficiency and coherence. When \( s \) is large enough to eliminate overlap, the process becomes a \emph{divide-and-conquer} strategy~\cite{li2024survey,yin2023nuwa}, where windows are synthesized independently. Conversely, smaller strides enforce stronger dependencies between windows due to larger overlapping regions. In the extreme case of \( s = 1 \), maximum coherence is achieved as nearly all timesteps are shared between consecutive windows. The optimal stride depends on the nature of the time series. Smaller strides ensure better alignment for signals with strong temporal dependencies, while larger strides may suffice for weaker ones. This flexibility allows our method to adapt to varying degrees of temporal dependence, ensuring an efficient and coherent synthesis of the generated signal.

% \begin{figure*}
%     \begin{subfigure}{0.3\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{images/ctype.pdf}
%         \caption{R}
%         \label{fig:c}
%     \end{subfigure}
%     \begin{subfigure}{0.3\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{images/mtype.pdf}
%         \caption{I}
%         \label{fig:m}
%     \end{subfigure}
%     \begin{subfigure}{0.3\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{images/ftype.pdf}
%         \caption{B}
%         \label{fig:f}
%     \end{subfigure}
%     \caption{R, I, and B type constraints for AustraliaTourism.  order: Year$\rightarrow$Month$\rightarrow$State$\rightarrow$Region$\rightarrow$Purpose}
%     \label{fig:tasklevels}
% \end{figure*}

\subsubsection{Time Complexity and Speedup Analysis}
\label{subsubsec:speed}
Our approach substantially improves the generation speed compared to autoregressive methods due to the efficient utilization of parallelization. Following the notation in \hyperref[alg:synth]{Algorithm 2}, \(\frac{M - w}{s} \) determines the total number of windows in the dataset, where \( M \) is the time series length, \( w \) is the window size, and \( s \) is the stride. The autoregressive approach processes each window sequentially. For each window, the denoising process requires \( T \) steps, with each step having a time complexity of \(O (t_\theta(w))\). Here $t_{\theta}(w)$ is the cost of denoising one step of a window. Consequently, the total time for autoregressive synthesis scales as \( \mathcal{O}(T \cdot t_\theta(w) \cdot (M-w)/s) \).

In contrast, the parallel synthesis algorithm processes multiple windows simultaneously within each mini-batch of size \( b \). As a result, the total number of mini-batches required is \( \frac{M-w}{b \cdot s} \). For each mini-batch, the denoising process is carried out in parallel across \( T \) timesteps for all \( b \) windows. Parallelization significantly reduces the time, yielding an effective time complexity of \( \mathcal{O}(T \cdot t_\theta(w) \cdot \frac{M-w}{b \cdot s}) \). This analysis suggests an \emph{ideal speedup} factor of approximately $b$ over the autoregressive approach, representing an upper bound on performance under minimal communication overhead and optimal hardware utilization.

\subsubsection{Categorical Encoding for Auxiliary Levels}
Given the auxiliary feature levels, recurring auxiliary feature categories like days of the week and months exhibit periodic patterns over timesteps. We apply \emph{sine and cosine transformations} to capture this cyclic behavior, drawing inspiration from the positional encodings used in Transformers~\cite{vaswani2017attention}. Specifically, we map each category to an angle on the unit circle and then use the sine and cosine of the angle to encode the feature. Let \( A_l \) represent a categorical feature with \( K \) unique values, such as the days of the week, where \( K = 7 \). We map each category \( k \in \{0, 1, \dots, K-1\} \) to an angle \( \theta_k = \frac{2 \pi k}{K} \) on the unit circle. Each categorical value \( k \) is then encoded by the coordinates \( (\sin(\theta_k), \cos(\theta_k)) \), reflecting the feature’s cyclical nature. This encoding captures the periodicity of the data, as both functions repeat smoothly over the circle. 

This approach offers a couple of practical advantages compared to one-hot encoding. First, it reduces the dimensionality of categorical features to just two values, regardless of the number of categories \( K \). In comparison, one-hot encoding would require \( K \) dimensions, which can become inefficient for large \( K \). Second, by leveraging the continuous, cyclical structure of sine and cosine, the encoding naturally captures dependencies within periodic data without needing the full expansion of one-hot encoding.





==> tables/ablation-encoding.tex <==
\begin{table}[htb]
    \centering
    \caption{Comparison of Encoding Schemes on (MSE) and Model Input Sizes Under Different Task Types.}
    \scalebox{.85}{
    \begin{tabular}{ll llll}
        \bottomrule
        \Xhline{1.5pt}
        % Top row: Dataset headers
        
        % Second row: Masking type headers for each dataset
         & \textbf{Method} & \bemph{R} & \bemph{I} & \bemph{B} & \textbf{In-dim}\\
         \cmidrule(lr){2-6}
        
        \multirow{2}{*}{MT}&OHE & $ 0.736_{ 0.021}$ & $ 0.652_{ 0.071}$ & $ 0.175_{ 0.014}$ & 79 \\
        
        % & $ 0.578 \pm \text{\scriptsize  0.008}$ & $ 0.568 \pm \text{\scriptsize  0.068}$ & $ 0.292 \pm \text{\scriptsize  0.012}$ \\

        % & ORD & $ 0.484 \pm \text{\scriptsize  0.074}$ & $ 0.124 \pm \text{\scriptsize  0.020}$ & $ 0.158 \pm \text{\scriptsize  0.016}$\\
        
        % & $ 0.477 \pm \text{\scriptsize  0.008}$ & $ 0.432 \pm \text{\scriptsize  0.045}$ & $ 0.249 \pm \text{\scriptsize  0.019}$ \\

        &CYC & $ \mathbf{0.512_{ 0.009}}$ & $ \mathbf{0.396_{ 0.019}}$ & $ \mathbf{0.111_{ 0.008}}$ & \textbf{13} \\
        
        % & $ 0.626 \pm \text{\scriptsize  0.005}$ & $ 0.410 \pm \text{\scriptsize  0.019}$ & $ 0.237 \pm \text{\scriptsize  0.017}$ \\

        
        \bottomrule
        \multirow{2}{*}{PE} & OHE & $ \mathbf{0.901_{ 0.013}}$ & $ 0.778_{ 0.044}$ & $ 0.480_{ 0.004}$ & 80 \\
        % & ORD & $ 0.484 \pm \text{\scriptsize  0.074}$ & $ 0.124 \pm \text{\scriptsize  0.020}$ & $ 0.158 \pm \text{\scriptsize  0.016}$\\
        &CYC & $ 1.006_{ 0.013}$ & $ \mathbf{0.587_{ 0.128}}$ & $ \mathbf{0.165_{ 0.003}}$ & \textbf{14} \\
        \bottomrule

        \multirow{2}{*}{RS} & OHE & $ \mathbf{0.587_{ 0.013}}$ & $ 0.687_{ 0.021}$ & $ 0.213_{ 0.001}$ & 58 \\

        & CYC & $ 0.598_{ 0.006}$ & $ \mathbf{0.537_{ 0.023}}$ & $ \mathbf{0.149_{ 0.002}}$ & \textbf{10} \\
        
        \bottomrule
        \Xhline{1.5pt}
    \end{tabular}}
    \label{tab:comparison}
    \vspace{-5pt}
\end{table}

==> tables/results_tsdiff.tex <==
\begin{table}[htb]
\centering
\caption{\centering{{Comparison of performance (MSE$\downarrow$) of TSDiff under varying guidance strengths, for different datasets and tasks (\textit{R}/\textit{I}/\textit{B}). Best score is in bold and second-best is \underline{underlined}.}}}
\label{tab:tsdiffres}
\setlength{\tabcolsep}{3pt} % Reduce column spacing
\renewcommand{\arraystretch}{1.2} % Adjust row spacing
\fontsize{12}{15}\selectfont % Set font size (12pt with 15pt line spacing)

\scalebox{0.61}{
\begin{tabular}{lcccccccc}
\Xhline{1.5pt}
\textbf{} & \textbf{0.0} & \textbf{0.5} & \textbf{1.0} & \textbf{2.0} \\
\midrule
\phantom{AT} (\bemph{R}) & $ 1.469_{.002}$ & $ 1.223_{.007}$ & $ \underline{1.174_{.002}}$ & $ \mathbf{1.062_{.022}}$ \\
AT (\bemph{I}) & $ 1.964_{.020}$ & $ \underline{1.480_{.003}}$ & $ \mathbf{1.395_{.020}}$ & $ 1.932_{.002}$ \\
\phantom{AT} (\bemph{B}) & $ \mathbf{1.331_{.012}}$ & $ 1.567_{.032}$ & $ \underline{1.446_{.007}}$ & $ 1.609_{.004}$ \\
\rowcolor{mygray}
\phantom{MT} (\bemph{R}) & $ 1.026_{.011}$ & $ \underline{0.964_{.009}}$ & $ \mathbf{0.880_{.014}}$ & $ 1.017_{.007}$ \\
\rowcolor{mygray}
MT (\bemph{I}) & $ \mathbf{0.573_{.036}}$ & $ \underline{0.768_{.027}}$ & $ 0.846_{.073}$ & $ 0.809_{.041}$ \\
\rowcolor{mygray}
\phantom{MT} (\bemph{B}) & $ \underline{0.215_{.008}}$ & $ \mathbf{0.200_{.010}}$ & $ 0.292_{.012}$ & $ 0.267_{.006}$ \\
\phantom{BQ} (\bemph{R}) & $ 2.333_{.014}$ & $ \mathbf{1.763_{.017}}$ & $ 2.444_{.010}$ & $ \underline{2.158_{.009}}$ \\
BQ (\bemph{I}) & $ \mathbf{1.342_{.011}}$ & $ \underline{1.422_{.025}}$ & $ 2.780_{.016}$ & $ 1.514_{.010}$ \\
\phantom{BQ} (\bemph{B}) & $ 0.244_{.022}$ & $ \mathbf{0.162_{.007}}$ & $ 0.167_{.007}$ & $ \underline{0.164_{.012}}$ \\
\rowcolor{mygray}
\phantom{RS} (\bemph{R}) & $ 0.785_{.008}$ & $ 0.893_{.021}$ & $ \mathbf{0.688_{.007}}$ & $ \underline{0.760_{.011}}$ \\
\rowcolor{mygray}
RS (\bemph{I}) & $ 0.971_{.037}$ & $ 0.827_{.032}$ & $ \underline{0.723_{.007}}$ & $ \mathbf{0.637_{.025}}$ \\
\rowcolor{mygray}
\phantom{RS} (\bemph{B}) & $ \underline{0.298_{.006}}$ & $ 0.458_{.011}$ & $ \mathbf{0.276_{.004}}$ & $ 0.394_{.007}$ \\
\phantom{PE} (\bemph{R}) & $ \mathbf{1.405_{.011}}$ & $ 1.667_{.005}$ & $ 2.105_{.003}$ & $ \underline{1.410_{.008}}$ \\
PE (\bemph{I}) & $ 2.171_{.092}$ & $ \mathbf{1.179_{.061}}$ & $ \underline{1.798_{.033}}$ & $ 2.538_{.039}$ \\
\phantom{PE} (\bemph{B}) & $ \mathbf{0.369_{.001}}$ & $ 0.469_{.002}$ & $ \underline{0.407_{.001}}$ & $ 0.469_{.001}$ \\
\midrule
Avg. & \underline{1.099} & \textbf{1.002} & 1.161 & 1.116\\
\Xhline{1.5pt}
\end{tabular}}
\end{table}
